MemorySeg: Online LiDAR Semantic Segmentation with a Latent Memory

Semantic segmentation of LiDAR point clouds has been widely studied in recent years, with most existing methods focusing on tackling this task using a single scan of the environment. However, leveraging the temporal stream of observations can provide very rich contextual information on regions of the scene with poor visibility (e.g., occlusions) or sparse observations (e.g., at long range), and can help reduce redundant computation frame after frame. In this paper, we tackle the challenge of exploiting the information from the past frames to improve the predictions of the current frame in an online fashion. To address this challenge, we propose a novel framework for semantic segmentation of a temporal sequence of LiDAR point clouds that utilizes a memory network to store, update and retrieve past information. Our framework also includes a regularizer that penalizes prediction variations in the neighborhood of the point cloud. Prior works have attempted to incorporate memory in range view representations for semantic segmentation, but these methods fail to handle occlusions and the range view representation of the scene changes drastically as agents nearby move. Our proposed framework overcomes these limitations by building a sparse 3D latent representation of the surroundings. We evaluate our method on SemanticKITTI, nuScenes, and PandaSet. Our experiments demonstrate the effectiveness of the proposed framework compared to the state-of-the-art.

==> figs/ablation_apm_k_table.tex <==
    \begin{table}[h]
        \begin{center}
        \scalebox{0.9}
        {
        \begin{tabular}{l|cccc|c}
        \hline %\hline %\\
        & class A & class B & class C & class D & mIoU \\
        \hline \hline
        k=3 & - & - & - & - & - \\
        k=5 & - & - & - & - & 70.8 \\
        k=8 & - & - & - & - & - \\
        \hline
        \end{tabular}
        }
        \end{center}
        \caption{Ablation on the padding neighborhood size in APM. Metrics are mIoU on the validation set provided in [\%]. \thomas{this will very likely go to supp}}
        \label{tab:padding}
        \end{table}

==> figs/nusc_val_table.tex <==
\begin{table*}[t]
    {%\Huge
    \centering
    \resizebox{\textwidth}{!}{
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|cc|cccccccccccccccc}
    \hline 
    \textbf{Method}  
    & \begin{sideways} \textbf{mIoU} \end{sideways} 
    & \begin{sideways} \textbf{FW-mIoU} \end{sideways} 
    & \begin{sideways} Barrier \end{sideways} 
    & \begin{sideways} Bicycle \end{sideways} 
    & \begin{sideways} Bus \end{sideways} 
    & \begin{sideways} Car \end{sideways} 
    & \begin{sideways} Construction \end{sideways} 
    & \begin{sideways} Motorcycle \end{sideways} 
    & \begin{sideways} Pedestrain \end{sideways} 
    & \begin{sideways} Traffic Cone \end{sideways} 
    & \begin{sideways} Trailer \end{sideways} 
    & \begin{sideways} Truck \end{sideways} 
    & \begin{sideways} Drivable \end{sideways} 
    & \begin{sideways} Other Flat \end{sideways} 
    & \begin{sideways} Sidewalk \end{sideways} 
    & \begin{sideways} Terrain \end{sideways} 
    & \begin{sideways} Manmade \end{sideways} 
    & \begin{sideways} Vegetation \end{sideways}  \\ 
    \hline
    RangeNet++ \cite{milioto2019rangenet++} & $65.5$ & $-$ & $66.0$ & $21.3$ & $77.2$ & $80.9$ & $30.2$ & $66.8$ & $69.6$ & $52.1$ & $54.2$ & $72.3$ & $94.1$ & $66.6$ & $63.5$ & $70.1$ & $83.1$ & $79.8$ \\
    PolarNet \cite{zhang2020polarnet} & $71.0$ & $-$ & $74.7$ & $28.2$ & $85.3$ & $90.9$ & $35.1$ & $77.5$ & $71.3$ & $58.8$ & $57.4$ & $76.1$ & $96.5$ & $71.1$ & $74.7$ & $74.0$ & $87.3$ & $85.7$ \\
    Salsanext \cite{cortinhal2020salsanext} & $72.2$ & $-$ & $74.8$ & $34.1$ & $85.9$ & $88.4$ & $42.2$ & $72.4$ & $72.2$ & $63.1$ & $61.3$ & $76.5$ & $96.0$ & $70.8$ & $71.2$ & $71.5$ & $86.7$ & $84.4$ \\
    Cylinder3D \cite{zhu2021cylindrical} & $76.1$ & $-$ &  $76.4$ & $40.3$ & $91.2$ & $\mathbf{93.8}$ & $51.3$ & $78.0$ & $78.9$ & $64.9$ & $62.1$ & $84.4$ & $96.8$ & $71.6$ & $\mathbf{76.4}$ & $75.4$ & $90.5$ & $87.4$ \\
    RPVNet \cite{xu2021rpvnet} & $77.6$ & $-$ & $78.2$ & $43.4$ & $92.7$ & $93.2$ & $49.0$ & $85.7$ & $80.5$ & $66.0$ & $66.9$ & $84.0$ & $96.9$ & $73.5$ & $75.9$ & $\mathbf{76.0}$ & $90.6$ & $88.9$ \\
    % PolarNet & 71.00 & \\
    % SalsaNext & 72.2 & \\
    % Cylinder3D & 76.1 & \\
    % % AMVNet & 77.2 & \\
    % RPVNet & 77.6 & \\
    % LiDARMultiNet & 82.0 & \\
    \hline
    SFB & 76.7 & 89.2 & 77.6 & 42.0 & 92.7 & 92.5 & 44.7 & 83.8 & 79.1 & 65.1 & 66.2 & 81.6 & 96.7 & 75.9 & 75.1 & 75.2 & 90.2 & 88.7 \\
    \proposed \ [ours] & $\mathbf{81.1}$ & $\mathbf{90.0}$ & $\mathbf{78.8}$ & $\mathbf{57.0}$ & $\mathbf{95.2}$ & 92.9 & $\mathbf{60.0}$ & $\mathbf{89.3}$ & $\mathbf{86.3}$ & $\mathbf{70.8}$ & $\mathbf{73.8}$ & $\mathbf{87.2}$ & $\mathbf{96.9}$ & $\mathbf{76.4}$ & 75.8 & 75.3 & $\mathbf{91.5}$ & $\mathbf{89.8}$ \\
    \hline
    \end{tabular}
    }
    \caption{Comparison to the state-of-the-art methods on the validation set of nuScenes \cite{caesar2020nuscenes} LiDAR semantic segmentation benchmark. We include LiDAR-only published approaches that report their validation mIoU. Metrics are provided in [\%].}
    \label{tab:nusc} }
    \end{table*} 

==> figs/sk_multi_val_table.tex <==
\begin{table*}[h]
    {%\Huge
    \centering
    \resizebox{\textwidth}{!}{
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|ccccccccccccccccccccccccc}
    \hline 
    \textbf{Method}  
    & \begin{sideways} \textbf{mIoU} \end{sideways} 
    & \begin{sideways} Car \end{sideways} 
    & \begin{sideways} Bicycle \end{sideways} 
    & \begin{sideways} Motorcycle \end{sideways} 
    & \begin{sideways} Truck \end{sideways} 
    & \begin{sideways} Other Vehicle \end{sideways} 
    & \begin{sideways} Person \end{sideways} 
    & \begin{sideways} Bicyclist \end{sideways} 
    & \begin{sideways} Motorcyclist \end{sideways} 
    & \begin{sideways} Road \end{sideways} 
    & \begin{sideways} Parking \end{sideways} 
    & \begin{sideways} Sidewalk \end{sideways} 
    & \begin{sideways} Other Ground \end{sideways} 
    & \begin{sideways} Building \end{sideways} 
    & \begin{sideways} Fence \end{sideways} 
    & \begin{sideways} Vegetation \end{sideways} 
    & \begin{sideways} Trunk \end{sideways} 
    & \begin{sideways} Terrain \end{sideways} 
    & \begin{sideways} Pole \end{sideways} 
    & \begin{sideways} Traffic Sign \end{sideways} 
    & \begin{sideways} car (m) \end{sideways} 
    & \begin{sideways} bicyclist (m) \end{sideways} 
    & \begin{sideways} person (m) \end{sideways} 
    & \begin{sideways} motorcyclist (m) \end{sideways} 
    & \begin{sideways} other-vehicle (m) \end{sideways} 
    & \begin{sideways} truck (m) \end{sideways} \\ 
    \hline
    5FB & 53.5 & 95.4 & 56.0 & 75.6 & 74.5 & 53.5 & $\mathbf{25.5}$ & 0.0 & 0.0 & 92.7 & 46.6 & 78.8 & 0.5 & 90.1 & 58.6 & 89.2 & 72.8 & 75.3 & 66.2 & $\mathbf{53.7}$ & $\mathbf{78.6}$ & 87.2 & 64.6 & 0.0 & 3.4 & 0.0 \\
    \proposed & $\mathbf{58.5}$ & $\mathbf{95.9}$ & $\mathbf{64.8}$ & $\mathbf{86.2}$ & $\mathbf{96.3}$ & $\mathbf{66.4}$ & $23.7$ & $0.0$ & $0.0$ & $\mathbf{95.5}$ & $\mathbf{55.7}$ & $\mathbf{83.9}$ & $\mathbf{5.0}$ & $\mathbf{91.4}$ & $\mathbf{62.7}$ & $\mathbf{89.7}$ & $\mathbf{73.9}$ & $\mathbf{78.1}$ & $\mathbf{66.7}$ & $52.1$ & $72.7$ & $\mathbf{94.4}$ & $\mathbf{72.0}$ & $0.0$ & $\mathbf{35.7}$ & $0.0$ \\
    \hline
    \end{tabular}
    }
    \caption{Comparison to our 5-frame baseline (5FB) on the validation set of SemanticKITTI \cite{behley2019semantickitti}. Movable actors are further divided into moving and static. Metrics are provided in [\%].}
    \label{tab:sk_multi_val} }
    \end{table*} 

==> figs/sk_single_test_miou_table.tex <==
\begin{table}[ht]
    \begin{center}
        \scalebox{0.7}
        {
    \begin{tabular}{l|c}
    \hline 
    \textbf{Method}  
    & \textbf{mIoU} \\ 
    \hline \hline
    % (AF)2S3-Net \cite{cheng20212} & $69.7$ & $94.5$ & $65.4$ & $86.8$ & $39.2$ & $41.1$ & $80.7$ & $80.4$ & $74.3$ & $91.3$ & $68.8$ & $72.5$ & $53.5$ & $87.9$ & $63.2$ & $70.2$ & $68.5$ & $53.7$ & $61.5$ & $71.0$ \\
    % RPVNet \cite{xu2021rpvnet} & $70.3$ & $97.6$ & $68.4$ & $68.7$ & $44.2$ & $61.1$ & $75.9$ & $74.4$ & $73.4$ & $93.4$ & $70.3$ & $80.7$ & $33.3$ & $93.5$ & $72.1$ & $86.5$ & $75.1$ & $71.7$ & $64.8$ & $61.4$ \\
    % 2DPASS \cite{yan20222dpass} & $72.9$ & $97.0$ &  $63.6$ & $63.4$ & $61.1$ & $61.5$ & $77.9$ & $81.3$ & $74.1$ & $89.7$ & $67.4$ & $74.7$ &  $40.0$ & $93.5$  & $72.9$ &$86.2$ & $73.9$ &  $71.0$ & $65.0$ & $70.4$ \\
    % \hline
    PointNet \cite{qi2017pointnet} & $14.6$ \\
    RangeNet++ \cite{milioto2019rangenet++} & $52.2$ \\
    RandLANet \cite{hu2020randla} & $53.9$ \\
    PolarNet \cite{zhang2020polarnet} & $54.3$ \\
    SqueezeSegv3 \cite{xu2020squeezesegv3} & $55.9$ \\
    TemporalLidarSeg\cite{duerr2020lidar} & $58.2$ \\
    KPConv \cite{thomas2019kpconv} & $58.8$ \\
    SalsaNext \cite{cortinhal2020salsanext} & $59.5$ \\
    Meta-RangeSeg \cite{wang2022meta} & 61.0 \\
    FusionNet \cite{zhang12356deep} & $61.3$  \\
    TornadoNet \cite{gerdzhev2021tornadonet} & $63.1$ \\
    % AMVNet & $65.3$ & $96.2$ & $59.9$ & $54.2$ & $48.8$ & $45.7$ & $71.0$ & $65.7$ & $11.0$ & $90.1$ & $71.0$ & $75.8$ & $32.4$ & $92.4$ & $69.1$ & $85.6$ & $71.7$ & $69.6$ & $62.7$ & $67.2$ \\
    % SPVCNN \cite{tang2020searching} & $63.8$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
    SPVNAS \cite{tang2020searching} & $67.0$ \\
    Cylinder3D \cite{zhu2021cylindrical} & $67.8$ \\
    (AF)2S3-Net \cite{cheng20212} & $69.7$ \\
    RPVNet \cite{xu2021rpvnet} & $70.3$ \\
    % PVKD \cite{hou2022pvkd} & $68.9$ & $96.7$ & $66.4$ & $61.0$ & $60.0$ & $59.3$ & $73.2$ & $72.1$ & $25.0$ & $91.4$ & $66.5$ & $76.2$ & $37.1$ & $93.0$ & $70.5$ & $85.9$ & $72.7$ & $69.8$ & $64.1$ & $67.8$ \\
    PVKD \cite{hou2022pvkd} & $71.2$ \\
    \hline
    % \proposed \ [ours] & 69.1 & 97.1 & 66.1 & 64.3 & 55.6 & 61.0 & 73.2 & 73.1 & 42.6 & 89.5 & 66.0 & 73.8 & 30.7 & 91.7 & 67.7 & 84.7 & 73.3 & 69.3 & 65.3 & 68.3 \\
    \proposed \ [ours] & $\mathbf{71.3}$ \\
    \hline
    \end{tabular}
    }
    \caption{Comparison to the state-of-the-art methods on the test set of SemanticKITTI \cite{behley2019semantickitti} single-scan benchmark. 
    % Note that we only include online approaches using the available LiDAR sweeps in the dataset without external data for fair comparison. 
    We include LiDAR-only published approaches at the time of submission. Metrics are provided in [\%]. A detailed breakdown of the IoU per class can be found in the supplementary material. 
    \raquel{bold the best performing to easy the reader}}
    \label{tab:skitti_single}
\end{center}
    \end{table} 

==> figs/sk_single_test_table.tex <==
% \begin{table*}[ht]
%     {%\Huge
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|ccc|c|ccccccccccccccccccc}
%     \hline 
%     \textbf{Method}  
%     & T & E & P
%     & \begin{sideways} \textbf{mIoU} \end{sideways} 
%     & \begin{sideways} Car \end{sideways} 
%     & \begin{sideways} Bicycle \end{sideways} 
%     & \begin{sideways} Motorcycle \end{sideways} 
%     & \begin{sideways} Truck \end{sideways} 
%     & \begin{sideways} Other Vehicle \end{sideways} 
%     & \begin{sideways} Person \end{sideways} 
%     & \begin{sideways} Bicyclist \end{sideways} 
%     & \begin{sideways} Motorcyclist \end{sideways} 
%     & \begin{sideways} Road \end{sideways} 
%     & \begin{sideways} Parking \end{sideways} 
%     & \begin{sideways} Sidewalk \end{sideways} 
%     & \begin{sideways} Other Ground \end{sideways} 
%     & \begin{sideways} Building \end{sideways} 
%     & \begin{sideways} Fence \end{sideways} 
%     & \begin{sideways} Vegetation \end{sideways} 
%     & \begin{sideways} Trunk \end{sideways} 
%     & \begin{sideways} Terrain \end{sideways} 
%     & \begin{sideways} Pole \end{sideways} 
%     & \begin{sideways} Traffic Sign \end{sideways} \\ 
%     \hline
%     Cylinder3D \cite{zhou2020cylinder3d} & x & - & - & $67.8$ & $97.1$ & $67.6$ & $64.0$ & $59.0$ & $58.6$ & $73.9$ & $67.9$ & $36.0$ & $91.4$ & $65.1$ & $75.5$ & $32.3$ & $91.0$ & $66.5$ & $85.4$ & $71.8$ & $68.5$ & $62.6$ & $65.6$ \\
%     (AF)2S3-Net \cite{cheng20212} & - & - & x & $69.7$ & $94.5$ & $65.4$ & $86.8$ & $39.2$ & $41.1$ & $80.7$ & $80.4$ & $74.3$ & $91.3$ & $68.8$ & $72.5$ & $53.5$ & $87.9$ & $63.2$ & $70.2$ & $68.5$ & $53.7$ & $61.5$ & $71.0$ \\
%     RPVNet \cite{xu2021rpvnet} & - & x & - & $70.3$ & $97.6$ & $68.4$ & $68.7$ & $44.2$ & $61.1$ & $75.9$ & $74.4$ & $73.4$ & $93.4$ & $70.3$ & $80.7$ & $33.3$ & $93.5$ & $72.1$ & $86.5$ & $75.1$ & $71.7$ & $64.8$ & $61.4$ \\
%     2DPASS \cite{yan20222dpass} & x & - & - & $72.9$ & $97.0$ &  $63.6$ & $63.4$ & $61.1$ & $61.5$ & $77.9$ & $81.3$ & $74.1$ & $89.7$ & $67.4$ & $74.7$ &  $40.0$ & $93.5$  & $72.9$ &$86.2$ & $73.9$ &  $71.0$ & $65.0$ & $70.4$ \\
%     \hline
%     PointNet \cite{qi2017pointnet} & - & - & - & $14.6$ & $46.3$ & $1.3$ & $0.3$ & $0.1$ & $0.8$ & $0.2$ & $0.2$ & $0.0$ & $61.6$ & $15.8$ & $35.7$ & $1.4$ & $41.4$ & $12.9$ & $31.0$ & $4.6$ & $17.6$ & $2.4$ & $3.7$ \\
%     RangeNet++ \cite{milioto2019rangenet++} & - & - & - & $52.2$ & $91.4$ & $25.7$ & $34.4$ & $25.7$ & $23.0$ & $38.3$ & $38.8$ & $4.8$ & $91.8$ & $65.0$ & $75.2$ & $27.8$ & $87.4$ & $58.6$ & $80.5$ & $55.1$ & $64.6$ & $47.9$ & $55.9$ \\
%     RandLANet \cite{hu2020randla} & - & - & - & $53.9$ & $94.2$ & $26.0$ & $25.8$ & $40.1$ & $38.9$ & $49.2$ & $48.2$ & $7.2$ & $90.7$ & $60.3$ & $73.7$ & $20.4$ & $86.9$ & $56.3$ & $81.4$ & $61.3$ & $66.8$ & $49.2$ & $47.7$ \\
%     PolarNet \cite{zhang2020polarnet} & - & - & -  & $54.3$ & $93.8$ & $40.3$ & $30.1$ & $22.9$ & $28.5$ & $43.2$ & $40.2$ & $5.6$ & $90.8$ & $61.7$ & $74.4$ & $21.7$ & $90.0$ & $61.3$ & $84.0$ & $65.5$ & $67.8$ & $51.8$ & $57.5$ \\
%     SqueezeSegv3 \cite{xu2020squeezesegv3} & - & - & -  & $55.9$ & $92.5$ & $38.7$ & $36.5$ & $29.6$ & $33.0$ & $45.6$ & $46.2$ & $20.1$ & $91.7$ & $63.4$ & $74.8$ & $26.4$ & $89.0$ & $59.4$ & $82.0$ & $58.7$ & $65.4$ & $49.6$ & $58.9$ \\
%     KPConv \cite{thomas2019kpconv} & - & - & -  & $58.8$ & $96.0$ & $30.2$ & $42.5$ & $33.4$ & $44.3$ & $61.5$ & $61.6$ & $11.8$ & $88.8$ & $61.3$ & $72.7$ & $31.6$ & $90.5$ & $64.2$ & $84.8$ & $69.2$ & $69.1$ & $56.4$ & $47.4$ \\
%     SalsaNext \cite{cortinhal2020salsanext} & - & - & -  & $59.5$ & $91.9$ & $48.3$ & $38.6$ & $38.9$ & $31.9$ & $60.2$ & $59.0$ & $19.4$ & $91.7$ & $63.7$ & $75.8$ & $29.1$ & $90.2$ & $64.2$ & $81.8$ & $63.6$ & $66.5$ & $54.3$ & $62.1$ \\
%     FusionNet \cite{zhang12356deep} & - & - & - & $61.3$ & $95.3$ & $47.5$ & $37.7$ & $41.8$ & $34.5$ & $59.5$ & $56.8$ & $11.9$ & $91.8$ & $68.8$ & $77.1$ & $30.8$ & $92.5$ & $69.4$ & $84.5$ & $69.8$ & $68.5$ & $60.4$ & $66.5$ \\
%     TornadoNet \cite{gerdzhev2021tornadonet} & - & - & - & $63.1$ & $94.2$ & $55.7$ & $48.1$ & $40.0$ & $38.2$ & $63.6$ & $60.1$ & $34.9$ & $89.7$ & $66.3$ & $74.5$ & $28.7$ & $91.3$ & $65.6$ & $85.6$ & $67.0$ & $71.5$ & $58.0$ & $65.9$ \\
%     % AMVNet & $65.3$ & $96.2$ & $59.9$ & $54.2$ & $48.8$ & $45.7$ & $71.0$ & $65.7$ & $11.0$ & $90.1$ & $71.0$ & $75.8$ & $32.4$ & $92.4$ & $69.1$ & $85.6$ & $71.7$ & $69.6$ & $62.7$ & $67.2$ \\
%     % SPVCNN \cite{tang2020searching} & $63.8$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
%     SPVNAS \cite{tang2020searching} & - & - & - & $67.0$ & $97.2$ & $50.6$ & $50.4$ & $56.6$ & $58.0$ & $67.4$ & $67.1$ & $50.3$ & $90.2$ & $67.6$ & $75.4$ & $21.8$ & $91.6$ & $66.9$ & $86.1$ & $73.4$ & $71.0$ & $64.3$ & $67.3$ \\
%     PVKD \cite{hou2022pvkd} & - & - & - & $68.9$ & $96.7$ & $66.4$ & $61.0$ & $60.0$ & $59.3$ & $73.2$ & $72.1$ & $25.0$ & $91.4$ & $66.5$ & $76.2$ & $37.1$ & $93.0$ & $70.5$ & $85.9$ & $72.7$ & $69.8$ & $64.1$ & $67.8$ \\
%     \hline
%     \proposed \ [ours] & - & - & - & 69.1 & 97.1 & 66.1 & 64.3 & 55.6 & 61.0 & 73.2 & 73.1 & 42.6 & 89.5 & 66.0 & 73.8 & 30.7 & 91.7 & 67.7 & 84.7 & 73.3 & 69.3 & 65.3 & 68.3 \\
%     \hline
%     \end{tabular}
%     }
%     \caption{Comparison to the state-of-the-art methods on the test set of SemanticKITTI \cite{behley2019semantickitti} single-scan challenge. Metrics are provided in [\%]. T: test-time augmentation ensembling. E: extra training data used. P: pseudo-labeling used.}
%     \label{tab:skitti_single_tep} }
%     \end{table*} 
\paragraph{SemanticKITTI single-scan results}
Tab.~\ref{tab:skitti_single} compares \proposed \ with state-of-the-art approaches on the test set of SemanticKITTI single-scan benchmark. This is a more competitive benchmark focusing on single-scan semantic segmentation where previous research has focused on proposing various architectures \cite{cheng20212,xu2021rpvnet,zhu2021cylindrical} or knowledge distillation techniques \cite{hou2022pvkd}. Our results show that \proposed{} can still outperform these methods, which are highly optimized for this benchmark. Tab.~\ref{tab:skitti_single_val_sota} compares our apporach with the others on the validation set of the same benchmark. Please note that most prior works have only reported the mIoU metric on the validation set. Therefore, we only included comparison of mIoU in this table but presented detailed class-wise IoUs in Tab.~\ref{tab:sk_val}.
\begin{table}[h]
    {%\Huge
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|ccccccccccccccccccc}
    \hline 
    \textbf{Method}  
    & \begin{sideways} \textbf{mIoU} \end{sideways} 
    & \begin{sideways} Car \end{sideways} 
    & \begin{sideways} Bicycle \end{sideways} 
    & \begin{sideways} Motorcycle \end{sideways} 
    & \begin{sideways} Truck \end{sideways} 
    & \begin{sideways} Other Vehicle \end{sideways} 
    & \begin{sideways} Person \end{sideways} 
    & \begin{sideways} Bicyclist \end{sideways} 
    & \begin{sideways} Motorcyclist \end{sideways} 
    & \begin{sideways} Road \end{sideways} 
    & \begin{sideways} Parking \end{sideways} 
    & \begin{sideways} Sidewalk \end{sideways} 
    & \begin{sideways} Other Ground \end{sideways} 
    & \begin{sideways} Building \end{sideways} 
    & \begin{sideways} Fence \end{sideways} 
    & \begin{sideways} Vegetation \end{sideways} 
    & \begin{sideways} Trunk \end{sideways} 
    & \begin{sideways} Terrain \end{sideways} 
    & \begin{sideways} Pole \end{sideways} 
    & \begin{sideways} Traffic Sign \end{sideways} \\ 
    \hline
    % (AF)2S3-Net \cite{cheng20212} & $69.7$ & $94.5$ & $65.4$ & $86.8$ & $39.2$ & $41.1$ & $80.7$ & $80.4$ & $74.3$ & $91.3$ & $68.8$ & $72.5$ & $53.5$ & $87.9$ & $63.2$ & $70.2$ & $68.5$ & $53.7$ & $61.5$ & $71.0$ \\
    % RPVNet \cite{xu2021rpvnet} & $70.3$ & $97.6$ & $68.4$ & $68.7$ & $44.2$ & $61.1$ & $75.9$ & $74.4$ & $73.4$ & $93.4$ & $70.3$ & $80.7$ & $33.3$ & $93.5$ & $72.1$ & $86.5$ & $75.1$ & $71.7$ & $64.8$ & $61.4$ \\
    % 2DPASS \cite{yan20222dpass} & $72.9$ & $97.0$ &  $63.6$ & $63.4$ & $61.1$ & $61.5$ & $77.9$ & $81.3$ & $74.1$ & $89.7$ & $67.4$ & $74.7$ &  $40.0$ & $93.5$  & $72.9$ &$86.2$ & $73.9$ &  $71.0$ & $65.0$ & $70.4$ \\
    % \hline
    PointNet \cite{qi2017pointnet} & $14.6$ & $46.3$ & $1.3$ & $0.3$ & $0.1$ & $0.8$ & $0.2$ & $0.2$ & $0.0$ & $61.6$ & $15.8$ & $35.7$ & $1.4$ & $41.4$ & $12.9$ & $31.0$ & $4.6$ & $17.6$ & $2.4$ & $3.7$ \\
    RangeNet++ \cite{milioto2019rangenet++} & $52.2$ & $91.4$ & $25.7$ & $34.4$ & $25.7$ & $23.0$ & $38.3$ & $38.8$ & $4.8$ & $91.8$ & $65.0$ & $75.2$ & $27.8$ & $87.4$ & $58.6$ & $80.5$ & $55.1$ & $64.6$ & $47.9$ & $55.9$ \\
    RandLANet \cite{hu2020randla} & $53.9$ & $94.2$ & $26.0$ & $25.8$ & $40.1$ & $38.9$ & $49.2$ & $48.2$ & $7.2$ & $90.7$ & $60.3$ & $73.7$ & $20.4$ & $86.9$ & $56.3$ & $81.4$ & $61.3$ & $66.8$ & $49.2$ & $47.7$ \\
    PolarNet \cite{zhang2020polarnet} & $54.3$ & $93.8$ & $40.3$ & $30.1$ & $22.9$ & $28.5$ & $43.2$ & $40.2$ & $5.6$ & $90.8$ & $61.7$ & $74.4$ & $21.7$ & $90.0$ & $61.3$ & $84.0$ & $65.5$ & $67.8$ & $51.8$ & $57.5$ \\
    SqueezeSegv3 \cite{xu2020squeezesegv3} & $55.9$ & $92.5$ & $38.7$ & $36.5$ & $29.6$ & $33.0$ & $45.6$ & $46.2$ & $20.1$ & $91.7$ & $63.4$ & $74.8$ & $26.4$ & $89.0$ & $59.4$ & $82.0$ & $58.7$ & $65.4$ & $49.6$ & $58.9$ \\
    TemporalLidarSeg\cite{duerr2020lidar} & $58.2$ & $94.1$ & $50.0$ & $45.7$ & $28.1$ & $37.1$ & $56.8$ & $47.3$ & $9.2$ & $91.7$ & $60.1$ & $75.9$ & $27.0$ & $89.4$ & $63.3$ & $83.9$ & $64.6$ & $66.8$ & $53.6$ & $60.5$ \\
    KPConv \cite{thomas2019kpconv} & $58.8$ & $96.0$ & $30.2$ & $42.5$ & $33.4$ & $44.3$ & $61.5$ & $61.6$ & $11.8$ & $88.8$ & $61.3$ & $72.7$ & $31.6$ & $90.5$ & $64.2$ & $84.8$ & $69.2$ & $69.1$ & $56.4$ & $47.4$ \\
    SalsaNext \cite{cortinhal2020salsanext} & $59.5$ & $91.9$ & $48.3$ & $38.6$ & $38.9$ & $31.9$ & $60.2$ & $59.0$ & $19.4$ & $91.7$ & $63.7$ & $75.8$ & $29.1$ & $90.2$ & $64.2$ & $81.8$ & $63.6$ & $66.5$ & $54.3$ & $62.1$ \\
    Meta-RangeSeg \cite{wang2022meta} & 61.0 & 93.9 & 50.1 & 43.8 & 43.9 & 43.2 & 63.7 & 53.1 & 18.7 & 90.6 & 64.3 & 74.6 & 29.2 & 91.1 & 64.7 & 82.6 & 65.5 & 65.5 & 56.3 & 64.2 \\
    FusionNet \cite{zhang12356deep} & $61.3$ & $95.3$ & $47.5$ & $37.7$ & $41.8$ & $34.5$ & $59.5$ & $56.8$ & $11.9$ & $91.8$ & $68.8$ & $77.1$ & $30.8$ & $\mathbf{92.5}$ & $\mathbf{69.4}$ & $84.5$ & $69.8$ & $68.5$ & $60.4$ & $66.5$ \\
    TornadoNet \cite{gerdzhev2021tornadonet} & $63.1$ & $94.2$ & $55.7$ & $48.1$ & $40.0$ & $38.2$ & $63.6$ & $60.1$ & $34.9$ & $89.7$ & $66.3$ & $74.5$ & $28.7$ & $91.3$ & $65.6$ & $85.6$ & $67.0$ & $71.5$ & $58.0$ & $65.9$ \\
    % AMVNet & $65.3$ & $96.2$ & $59.9$ & $54.2$ & $48.8$ & $45.7$ & $71.0$ & $65.7$ & $11.0$ & $90.1$ & $71.0$ & $75.8$ & $32.4$ & $92.4$ & $69.1$ & $85.6$ & $71.7$ & $69.6$ & $62.7$ & $67.2$ \\
    % SPVCNN \cite{tang2020searching} & $63.8$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
    SPVNAS \cite{tang2020searching} & $67.0$ & $97.2$ & $50.6$ & $50.4$ & $56.6$ & $58.0$ & $67.4$ & $67.1$ & $50.3$ & $90.2$ & $67.6$ & $75.4$ & $21.8$ & $91.6$ & $66.9$ & $86.1$ & $73.4$ & $71.0$ & $64.3$ & $67.3$ \\
    Cylinder3D \cite{zhu2021cylindrical} & $67.8$ & $97.1$ & $67.6$ & $64.0$ & $\mathbf{59.0}$ & $58.6$ & $73.9$ & $67.9$ & $36.0$ & $91.4$ & $65.1$ & $75.5$ & $32.3$ & $91.0$ & $66.5$ & $85.4$ & $71.8$ & $68.5$ & $62.6$ & $65.6$ \\
    (AF)2S3-Net \cite{cheng20212} & $69.7$ & $94.5$ & $65.4$ & $\mathbf{86.8}$ & $39.2$ & $41.1$ & $\mathbf{80.7}$ & $\mathbf{80.4}$ & $\mathbf{74.3}$ & $91.3$ & $68.8$ & $72.5$ & $\mathbf{53.5}$ & $87.9$ & $63.2$ & $70.2$ & $68.5$ & $53.7$ & $61.5$ & $\mathbf{71.0}$ \\
    RPVNet \cite{xu2021rpvnet} & $70.3$ & $\mathbf{97.6}$ & $\mathbf{68.4}$ & $68.7$ & $44.2$ & $\mathbf{61.1}$ & $\mathbf{75.9}$ & $74.4$ & $\mathbf{73.4}$ & $\mathbf{93.4}$ & $\mathbf{70.3}$ & $\mathbf{80.7}$ & $33.3$ & $\mathbf{93.5}$ & $\mathbf{72.1}$ & $\mathbf{86.5}$ & $\mathbf{75.1}$ & $\mathbf{71.7}$ & $64.8$ & $61.4$ \\
    % PVKD \cite{hou2022pvkd} & $68.9$ & $96.7$ & $66.4$ & $61.0$ & $60.0$ & $59.3$ & $73.2$ & $72.1$ & $25.0$ & $91.4$ & $66.5$ & $76.2$ & $37.1$ & $93.0$ & $70.5$ & $85.9$ & $72.7$ & $69.8$ & $64.1$ & $67.8$ \\
    PVKD \cite{hou2022pvkd} & $71.2$ & $97.0$ & $67.9$ & $\mathbf{69.3}$ & $53.5$ & $60.2$ & $75.1$ & $73.5$ & $50.5$ & $\mathbf{91.8}$ & $\mathbf{70.9}$ & $\mathbf{77.5}$ & $\mathbf{41.0}$ & $92.4$ & $69.4$ & $\mathbf{86.5}$ & $\mathbf{73.8}$ & $\mathbf{71.9}$ & $\mathbf{64.9}$ & $65.8$ \\
    \hline
    % \proposed \ [ours] & 69.1 & 97.1 & 66.1 & 64.3 & 55.6 & 61.0 & 73.2 & 73.1 & 42.6 & 89.5 & 66.0 & 73.8 & 30.7 & 91.7 & 67.7 & 84.7 & 73.3 & 69.3 & 65.3 & 68.3 \\
    \proposed \ [ours] & $\mathbf{71.3}$ & $\mathbf{97.4}$ & $\mathbf{68.1}$ & 69.1 & $\mathbf{58.7}$ & $\mathbf{65.7}$ & 75.2 & $\mathbf{76.4}$ & 56.2 & 89.8 & 65.6 & 74.8 & 32.1 & 91.9 & 67.8 & 85.2 & 73.7 & 70.5 & $\mathbf{66.4}$ & $\mathbf{70.1}$ \\
    \hline
    \end{tabular}
    }
    \caption{Comparison to the state-of-the-art methods on the test set of SemanticKITTI \cite{behley2019semantickitti} single-scan benchmark. 
    % Note that we only include online approaches using the available LiDAR sweeps in the dataset without external data for fair comparison. 
    We include LiDAR-only published approaches at the time of submission. Metrics are provided in [\%]. Top two entries of each classes are bolded. }
    \label{tab:skitti_single} }
    \end{table} 

==> figs/sk_single_val_table.tex <==
\begin{table}[h]
    \begin{center}
    \scalebox{0.9}
    {
    \begin{tabular}{l|ccc}
    \hline %\hline %\\
    \textbf{Method} & \textbf{mIoU}\\
    \hline \hline
    % PointNet \cite{qi2017pointnet} & x \\
    % RangeNet++ \cite{milioto2019rangenet++} & x\\
    RandLANet \cite{hu2020randla} & 57.1 \\
    PolarNet \cite{zhang2020polarnet} & 54.9 \\
    TornadoNet \cite{gerdzhev2021tornadonet} & 64.5 \\
    SPVNAS \cite{tang2020searching} & 64.7 \\
    Cylinder3D \cite{zhu2021cylindrical} & 65.9 \\
    PVKD \cite{hou2022pvkd} & 66.4 \\
    RPVNet \cite{xu2021rpvnet} & 69.6 \\
    \hline
    \proposed \ [ours] & 70.8 \\
    \proposed \ [ours] + TTA & 71.5 \\
    \hline
    \end{tabular}
    }
    \end{center}
    \caption{Comparison to the state-of-the-art methods on the validation set of SemanticKITTI \cite{behley2019semantickitti}. Metrics are provided in [\%].}
    \label{tab:skitti_single_val_sota}
    \end{table}

==> figs/sk_val_detail_table.tex <==
    \begin{table*}[t]
        {%\Huge
        \centering
        \resizebox{\textwidth}{!}{
        % \resizebox{\columnwidth}{!}{
        \begin{tabular}{l|c|ccccccccccccccccccc}
        \hline 
        \textbf{Method}  
        & \begin{sideways} \textbf{mIoU} \end{sideways} 
        & \begin{sideways} Car \end{sideways} 
        & \begin{sideways} Bicycle \end{sideways} 
        & \begin{sideways} Motorcycle \end{sideways} 
        & \begin{sideways} Truck \end{sideways} 
        & \begin{sideways} Other Vehicle \end{sideways} 
        & \begin{sideways} Person \end{sideways} 
        & \begin{sideways} Bicyclist \end{sideways} 
        & \begin{sideways} Motorcyclist \end{sideways} 
        & \begin{sideways} Road \end{sideways} 
        & \begin{sideways} Parking \end{sideways} 
        & \begin{sideways} Sidewalk \end{sideways} 
        & \begin{sideways} Other Ground \end{sideways} 
        & \begin{sideways} Building \end{sideways} 
        & \begin{sideways} Fence \end{sideways} 
        & \begin{sideways} Vegetation \end{sideways} 
        & \begin{sideways} Trunk \end{sideways} 
        & \begin{sideways} Terrain \end{sideways} 
        & \begin{sideways} Pole \end{sideways} 
        & \begin{sideways} Traffic Sign \end{sideways} \\ 
        \hline
        % (AF)2S3-Net \cite{cheng20212} & 74.2 \\
        % RPVNet \cite{xu2021rpvnet} & 69.6 \\
        % 2DPASS \cite{yan20222dpass} & 69.3 \\
        % \hline
        % PointNet \cite{qi2017pointnet} & x \\
        % RangeNet++ \cite{milioto2019rangenet++} & x\\
        % RandLANet \cite{hu2020randla} & 57.1 \\
        % PolarNet \cite{zhang2020polarnet} & 54.9 \\
        % TornadoNet \cite{gerdzhev2021tornadonet} & 64.5 \\
        % SPVNAS \cite{tang2020searching} & 64.7 \\
        % Cylinder3D \cite{zhu2021cylindrical} & 65.9 \\
        % PVKD \cite{hou2022pvkd} & 66.4 \\
        % RPVNet \cite{xu2021rpvnet} & 69.6 \\
        % \hline
        SFB w/o cutMix & 66.2 & 96.0 & 54.2 & 76.7 & 78.5 & 53.5 & 71.2 & 92.0 & 0.7 & 94.5 & 49.3 & 82.2 & 3.8 & 91.0 & 63.8 & 88.7 & 71.2 & 76.0 & 64.6 & 49.4 \\
        SFB & 67.2 & 96.9 & 60.0 & 79.5 & 76.9 & 67.0 & 74.0 & 91.2 & 1.6 & 94.5 & 49.4 & 82.0 & 6.1 & 90.6 & 61.0 & 88.0 & 69.0 & 74.4 & 64.8 & 50.8 \\
        % \hline
        M1 & 69.5 & 97.5 & 62.4 & 88.0 & 79.1 & 74.4 & 83.7 & 93.2 & 2.5 & 95.3 & 55.7 & 83.5 & 3.3 & 90.4 & 61.8 & 88.1 & 69.5 & 74.7 & 64.9 & 52.2 \\
        M2 & 69.7 & 97.6 & 58.4 & 86.2 & 94.5 & 77.8 & 83.1 & 94.0 & 0.0 & 94.9 & 54.5 & 83.0 & 3.9 & 90.9 & 63.5 & 87.3 & 68.8 & 71.5 & 65.1 & 50.0 \\
        M3 & 69.7 & 97.3 & 59.4 & 84.9 & 82.5 & 73.7 & 83.1 & 93.7 & 8.9 & 94.9 & 50.1 & 82.4 & 4.6 & 90.8 & 61.6 & 89.2 & 70.8 & 77.2 & 66.0 & 52.6 \\
        M4 [ours] & 70.8 & 97.4 & 61.5 & 89.1 & 93.0 & 76.2 & 83.6 & 95.0 & 0.3 & 95.3 & 52.4 & 83.0 & 7.5 & 91.4 & 64.1 & 89.3 & 73.6 & 77.2 & 65.6 & 50.4 \\
        M4 [ours] + TTA & $71.5$ & $97.9$ & $64.6$ & $89.3$ & $95.4$ & $81.9$ & $84.6$ & $95.2$ & $0.0$ & $95.6$ & $52.9$ & $83.9$ & $2.9$ & $91.3$ & $62.9$ & $89.7$ & $74.4$ & $77.8$ & $66.5$ & $51.8$ \\
        \hline
        \end{tabular}
        }
        \caption{Class-wise IoUs of our ablated methods on the validation set of SemanticKITTI \cite{behley2019semantickitti}. Metrics are provided in [\%].}
        \label{tab:sk_val} }
        \end{table*} 
        
            \begin{table*}[t]
                {%\Huge
                \centering
                \resizebox{\textwidth}{!}{
                % \resizebox{\columnwidth}{!}{
                \begin{tabular}{l|c|ccccccccccccccccccc}
                \hline 
                \textbf{Memory Vox Size}
                & \begin{sideways} \textbf{mIoU} \end{sideways} 
                & \begin{sideways} Car \end{sideways} 
                & \begin{sideways} Bicycle \end{sideways} 
                & \begin{sideways} Motorcycle \end{sideways} 
                & \begin{sideways} Truck \end{sideways} 
                & \begin{sideways} Other Vehicle \end{sideways} 
                & \begin{sideways} Person \end{sideways} 
                & \begin{sideways} Bicyclist \end{sideways} 
                & \begin{sideways} Motorcyclist \end{sideways} 
                & \begin{sideways} Road \end{sideways} 
                & \begin{sideways} Parking \end{sideways} 
                & \begin{sideways} Sidewalk \end{sideways} 
                & \begin{sideways} Other Ground \end{sideways} 
                & \begin{sideways} Building \end{sideways} 
                & \begin{sideways} Fence \end{sideways} 
                & \begin{sideways} Vegetation \end{sideways} 
                & \begin{sideways} Trunk \end{sideways} 
                & \begin{sideways} Terrain \end{sideways} 
                & \begin{sideways} Pole \end{sideways} 
                & \begin{sideways} Traffic Sign \end{sideways} \\ 
                \hline
                % (AF)2S3-Net \cite{cheng20212} & 74.2 \\
                % RPVNet \cite{xu2021rpvnet} & 69.6 \\
                % 2DPASS \cite{yan20222dpass} & 69.3 \\
                % \hline
                % PointNet \cite{qi2017pointnet} & x \\
                % RangeNet++ \cite{milioto2019rangenet++} & x\\
                % RandLANet \cite{hu2020randla} & 57.1 \\
                % PolarNet \cite{zhang2020polarnet} & 54.9 \\
                % TornadoNet \cite{gerdzhev2021tornadonet} & 64.5 \\
                % SPVNAS \cite{tang2020searching} & 64.7 \\
                % Cylinder3D \cite{zhu2021cylindrical} & 65.9 \\
                % PVKD \cite{hou2022pvkd} & 66.4 \\
                % RPVNet \cite{xu2021rpvnet} & 69.6 \\
                % \hline
                
                $v_m =$ 0.25 m & 70.2 & 97.1 & 65.4 & 89.4 & 90.3 & 69.2 & 78.1 & 94.9 & 2.4 & 95.2 & 53.9 & 83.1 & 4.9 & 91.3 & 63.2 & 89.3 & 69.8 & 77.1 & 65.3 & 53.7 \\
                $v_m =$ 0.5 m & 70.8 & 97.4 & 61.5 & 89.1 & 93.0 & 76.2 & 83.6 & 95.0 & 0.3 & 95.3 & 52.4 & 83.0 & 7.5 & 91.4 & 64.1 & 89.3 & 73.6 & 77.2 & 65.6 & 50.4 \\
                $v_m =$ 1.0 m & 70.1 & 97.2 & 59.2 & 84.8 & 91.5 & 74.2 & 79.4 & 93.7 & 0.3 & 95.1 & 55.4 & 82.5 & 14.5 & 90.7 & 61.3 & 88.7 & 71.5 & 76.1 & 64.2 & 50.9 \\
                $v_m =$ 2.0 m & 67.9 & 97.2 & 55.1 & 76.3 & 79.8 & 73.6 & 74.3 & 92.0 & 1.4 & 94.6 & 53.4 & 82.0 & 7.3 & 90.8 & 61.9 & 87.9 & 71.1 & 74.4 & 65.4 & 52.3 \\
                \hline
                \end{tabular}
                }
                \caption{Ablation results of different memory voxel size $v_m$ on the validation set of SemanticKITTI \cite{behley2019semantickitti}. Metrics are provided in [\%].}
                \label{tab:ab_mem_vox_size} }
                \end{table*} 

                \begin{table*}[t]
                    {%\Huge
                    \centering
                    \resizebox{\textwidth}{!}{
                    % \resizebox{\columnwidth}{!}{
                    \begin{tabular}{l|c|ccccccccccccccccccc}
                    \hline 
                    \textbf{APM Neighbours}
                    & \begin{sideways} \textbf{mIoU} \end{sideways} 
                    & \begin{sideways} Car \end{sideways} 
                    & \begin{sideways} Bicycle \end{sideways} 
                    & \begin{sideways} Motorcycle \end{sideways} 
                    & \begin{sideways} Truck \end{sideways} 
                    & \begin{sideways} Other Vehicle \end{sideways} 
                    & \begin{sideways} Person \end{sideways} 
                    & \begin{sideways} Bicyclist \end{sideways} 
                    & \begin{sideways} Motorcyclist \end{sideways} 
                    & \begin{sideways} Road \end{sideways} 
                    & \begin{sideways} Parking \end{sideways} 
                    & \begin{sideways} Sidewalk \end{sideways} 
                    & \begin{sideways} Other Ground \end{sideways} 
                    & \begin{sideways} Building \end{sideways} 
                    & \begin{sideways} Fence \end{sideways} 
                    & \begin{sideways} Vegetation \end{sideways} 
                    & \begin{sideways} Trunk \end{sideways} 
                    & \begin{sideways} Terrain \end{sideways} 
                    & \begin{sideways} Pole \end{sideways} 
                    & \begin{sideways} Traffic Sign \end{sideways} \\ 
                    \hline
                    k=3 & 69.7 & 97.2 & 61.3 & 84.8 & 90.8 & 73.5 & 74.5 & 92.8 & 3.5 & 95.2 & 52.2 & 82.9 & 6.1 & 91.6 & 64.2 & 88.4 & 73.4 & 75.0 & 65.2 & 52.1 \\
                    k=5 & 70.8 & 97.4 & 61.5 & 89.1 & 93.0 & 76.2 & 83.6 & 95.0 & 0.3 & 95.3 & 52.4 & 83.0 & 7.5 & 91.4 & 64.1 & 89.3 & 73.6 & 77.2 & 65.6 & 50.4 \\
                    k=8 & 70.0 & 97.3 & 59.7 & 84.8 & 93.7 & 75.1 & 79.9 & 94.0 & 0.4 & 94.9 & 54.2 & 82.6 & 6.4 & 91.4 & 63.0 & 88.7 & 72.0 & 75.8 & 64.9 & 51.7 \\
                    \hline
                    \end{tabular}
                    }
                    \caption{Ablation results of different padding neighbourhood sizes $k$ in APM on the validation set of SemanticKITTI \cite{behley2019semantickitti}. Metrics are provided in [\%].}
                    \label{tab:ab_mem_padding_size} }
                    \end{table*} 

==> sections/supp_ablations.tex <==
\section{Addtional Ablations}

==> sections/supp_qualitative.tex <==
\section{Additional Qualitative Results}
